Bounding the degrees of the defining equations of Rees rings for certain determinantal and Pfaffian ideals

We consider ideals of minors of a matrix, ideals of minors of a symmetric matrix, and ideals of Pfaffians of an alternating matrix. Assuming these ideals are of generic height, we characterize the condition $G_{s}$ for these ideals in terms of the heights of other ideals of minors or Pfaffians of the same matrix. We additionally obtain bounds on the generation and concentration degrees of the Rees rings of a subclass of such ideals via specialization of the Rees rings in the generic case. We do this by proving, given sufficient height conditions on ideals of minors or Pfaffians of the matrix, the specialization of a resolution of the Rees ring in the generic case is an approximate resolution of the Rees ring in question. We end the paper by giving some explicit generation and concentration degree bounds.

==> ourdefs.tex <==

\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\Coker}{Coker}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Id}{id}
\DeclareMathOperator{\MIN}{Min}
\DeclareMathOperator{\HEIGHT}{ht}
\DeclareMathOperator{\END}{End}
\DeclareMathOperator{\HOM}{Hom}
\DeclareMathOperator{\ANN}{ann}
\DeclareMathOperator{\JRAD}{rad}
\DeclareMathOperator{\SPEC}{Spec}
\DeclareMathOperator{\QUOT}{Quot}
\DeclareMathOperator{\ADJ}{Adj}
\DeclareMathOperator{\PFADJ}{PfAdj}
\DeclareMathOperator{\RANK }{rank}
\DeclareMathOperator{\ASS }{Ass}
\DeclareMathOperator{\SUPP}{Supp}
\DeclareMathOperator{\TOR}{Tor}
\DeclareMathOperator{\EXT}{Ext}
\DeclareMathOperator{\DEPTH }{depth}
\DeclareMathOperator{\GRADE }{grade}
\DeclareMathOperator{\PDIM}{pd}
\DeclareMathOperator{\ASGR}{gr}
\DeclareMathOperator{\SYM}{Sym}
\DeclareMathOperator{\ANC}{AN}
\DeclareMathOperator{\MON}{Mon}
\DeclareMathOperator{\FITT}{Fitt}
\DeclareMathOperator{\PFAFF}{Pf}
\DeclareMathOperator{\LCM}{lcm}
\DeclareMathOperator{\INITIDL}{in}
\DeclareMathOperator{\GIN}{gin}
\DeclareMathOperator{\REG}{reg}
\DeclareMathOperator{\TOPDEG}{topdeg}
\DeclareMathOperator{\CHAR}{char}
\DeclareMathOperator{\PROJ}{Proj}
\DeclareMathOperator{\trdeg}{trdeg}

\usetikzlibrary{positioning}

\mathchardef\mhyphen="2D

\newcommand{\paren }[1]{\left( #1 \right)}
\newcommand{\brak }[1]{\left[ #1 \right]}
\newcommand{\curly}[1]{\left\{ #1 \right\}}
\newcommand{\gradedcomp}[2]{\brak{#1}_{#2}}
\newcommand{\minof}[2][]{\min_{#1} \curly{#2}}
\newcommand{\maxof}[2][]{\max_{#1} \curly{#2}}
\newcommand{\supof}[2][]{\sup_{#1} \curly{#2}}
\newcommand{\infof}[2][]{\inf_{#1} \curly{#2}}

\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\bs}{\backslash}
\newcommand{\zs}{\{0\}}
\newcommand{\id}[1]{\Id_{#1}} %--
\newcommand{\Zn}[1]{\mathbb{Z}_{#1}} 

\newcommand{\Z}{\mathbb{Z}} 
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\End}[2]{\END_{#1}\! \left(#2\right)} %--
\newcommand{\fV}[2]{\left._{#1} #2 \right.} 
\newcommand{\Hom}[3]{\HOM_{#1}\! \left(#2, #3\right)} %--
\newcommand{\sHom}[3]{\mbox{\small Hom}_{#1}\!(#2, #3)}
\newcommand{\tHom}[3]{\mbox{\tiny Hom}_{#1}\!(#2, #3)}

\newcommand{\ann}[2]{\ANN_{#1}\!\left(#2\right)} %--
\newcommand{\rad}[1]{\JRAD\!\left(#1\right)} %--
\newcommand{\frk}[1]{\mathfrak{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}
\newcommand{\fm}{\mathfrak{m}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\chr}[1]{\CHAR #1}

\newcommand{\tors}[2]{\tau_{#1}\!\left(#2\right)}

\newcommand{\oplist}[4]{#1_{#2} #4 \cdots #4 #1_{#3}}
\newcommand{\eltlist}[3]{ #1_{#2}, \ldots, #1_{#3} }
\newcommand{\projcoords}[3]{ #1_{#2} : \cdots : #1_{#3} }
\newcommand{\projspace}[2]{\mathbb{P}^{#1}_{#2}}
\newcommand{\affspace}[2]{\mathbb{A}^{#1}_{#2}}
\newcommand{\poly}[2]{#1 \! \left[ #2 \right]}
\newcommand{\polyList}[4]{#1 \! \left[ \eltlist{#2}{#3}{#4} \right]}
\newcommand{\polySmall}[2]{#1 \left[ #2 \right]}
\newcommand{\polyListSmall}[4]{#1 \left[ \eltlist{#2}{#3}{#4} \right]}
\newcommand{\func}[2]{#1 \! \left( #2 \right)}
\newcommand{\funcSmall}[2]{#1 \left( #2 \right)}
\newcommand{\V}[1]{\func{V}{#1}}

\newcommand{\tensor}[3]{#1 \otimes_{#3} #2}
\newcommand{\obar}[1]{\overline{#1}}
\newcommand{\ubar}[1]{\underline{#1}}
\newcommand{\fibpr}[3]{#1 \underset{#3}{\cartprod} #2}
\newcommand{\sympow}[2]{#1^{(#2)}}
\newcommand{\mspec}[1]{\fm \mhyphen \SPEC \! \left(#1\right)} %--
\newcommand{\spec}[1]{\SPEC\!\left(#1\right)}
\newcommand{\Min}[1]{\MIN \! \left(#1 \right)}
\newcommand{\proj}[1]{\PROJ\!\left(#1\right)}
\newcommand{\quot}[1]{\QUOT\!\left(#1\right)} %--
\newcommand{\adj}[1]{\ADJ\!\left(#1\right)} %--
\newcommand{\pfadj}[1]{\PFADJ\!\left(#1\right)} %--
\newcommand{\rank}[1]{\RANK\!\left(#1\right)} %--
\newcommand{\gens}[2]{\mu_{#1}\!\left(#2\right)}
\newcommand{\gensSmall}[2]{\mu_{#1}\left(#2\right)}

\newcommand{\wtld}[1]{\widetilde{#1}}
\newcommand{\assP}[2]{\ASS_{#1}\!\left(#2\right)} %--
\newcommand{\colonideal}[3]{\left( #3 \underset{#1}{:} #2 \right)} 
\newcommand{\length}[2]{l_{#1}\!({#2})}
\newcommand{\supp}[2]{\SUPP_{#1}\!\left(#2\right) } %--
\newcommand{\fpow}[2]{#1^{(#2)}}
\newcommand{\restr}[2]{\left.#1\right|_{#2}}
\newcommand{\vpl}{\varprojlim}
\newcommand{\vil}{\varinvlim}


\newcommand{\Tor}[4]{\TOR_{#1}^{#2}\!\left(#3, #4\right)} %--
\newcommand{\Ext}[4]{\EXT_{#2}^{#1}\!\left(#3, #4\right)} %--
\newcommand{\comp}[2][\bullet]{\mathbf{#2}\!_{#1}}
\newcommand{\compp}[2][\bullet]{\mathbf{#2}_{#1}}
\newcommand{\cocomp}[2][\bullet]{\mathbf{#2}\!^{#1}}
\newcommand{\dirlim}{\varinjlim}
\newcommand{\invlim}{\varprojlim}

\newcommand{\depth}[2]{\DEPTH_{#1}  #2 } %--
\newcommand{\grade}[1]{\GRADE  #1 } %--
\newcommand{\gradeIM}[2]{\GRADE\!\left(#1, #2\right)}
\newcommand{\pdim}[2]{\PDIM_{#1}\!  #2 } %--
\newcommand{\hgt}[1]{\HEIGHT  #1 } %--
\newcommand{\asgr}[2]{\ASGR_{#1}\!\left(#2\right)} %--
\newcommand{\rees}[1]{\mathcal{R}\!\left(#1\right)}
\newcommand{\sym}[2]{\mathcal S_{#1}\!\left(#2\right)} %--
\newcommand{\Fcond}[1]{\mathcal{F}_{#1}}
\newcommand{\Gcond}[1]{G_{#1}}
\newcommand{\Gs}{\Gcond{s}}
\newcommand{\Gd}{\Gcond{d}}
\newcommand{\Gell}{\Gcond{\ell}}
\newcommand{\Ginf}{\Gcond{\infty}}
\newcommand{\ANcond}[1]{\ANC_{#1}} %--

\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\dcl}[1]{\mathfrak{Cl}\!\left(#1\right)}

\newcommand{\linked}[3]{#1 \underset{#3}{\sim} #2}
\newcommand{\link}[1]{\begin{smallmatrix} \\ \sim\\ \ubar{#1} \end{smallmatrix}} %New command for linking? Not perfect but better than before, I think.
\newcommand{\alf}{\alpha}

\newcommand{\ubx}{\ubar x}
\newcommand{\ubalf}{\ubar \alf}
\newcommand{\mcomp}[2]{\comp{\mathcal M_{#1}}{(#2)}}
\newcommand{\zcomp}[2]{\comp{\mathcal Z_{#1}}{(#2)}}
\newcommand{\bcomp}[2]{\comp{\mathcal B_{#1}}{(#2)}}

\newcommand{\resfld}[1]{\kappa\!\left(#1\right)}
\newcommand{\locoh}[3]{\mathrm{H}^{#1}_{#2}\hspace{-0.7mm}\left(#3\right)}
\newcommand{\secfunc}[2]{\Gamma_{#1}\!\left(#2\right)}
\newcommand{\vep}{\varepsilon}
\newcommand{\cont}[1]{ \left.^a #1 \right.}
\newcommand{\Mon}[1]{\MON\!\left( #1 \right) } %--
\newcommand{\sat}[1]{\widetilde{#1}}
\newcommand{\lcm}[2]{\LCM\!\left(#1,#2\right)}

\newcommand{\IN}[2]{\INITIDL_{#1}\!\left(#2\right)}
\newcommand{\spair}[2]{ \; S \! \left(#1,#2 \right)}
\newcommand{\gb}{Gr{\"o}bner }
\newcommand{\xa}[2]{\mathbf{#1}^{\underline{#2}}}
\newcommand{\bv}[1]{\mathbf{#1}}
\newcommand{\gin}[1]{\GIN\,\left(#1\right)}
\newcommand{\aspread}[1]{\ell \! \left( #1 \right)}
\newcommand{\detid}[2]{I_{#1}\!\left(#2\right)}
\newcommand{\pfaffid}[2]{\PFAFF_{#1}\!\left(#2\right)}

\newcommand{\fitt}[2]{\FITT_{#1}\!\left( #2 \right)}

\newcommand{\td}[1]{\TOPDEG #1}
\newcommand{\tdp}[1]{\TOPDEG \! \left( #1 \right)}
\newcommand{\dia}[1]{#1_{\diamond}}
\newcommand{\cartprod}{\hspace{-0.7 mm}\times \hspace{-0.9 mm}}
\newcommand{\A}[2]{\mcal{A}_{#1}\!\left(#2\right)}
\newcommand{\bzero}[1]{b_{0}\!\left(#1\right)}
\newcommand{\fiber}[1]{\mathcal{F}\hspace{-1mm}\left(#1\right)}
\newcommand{\hmgy}[2]{\mathrm{H}_{#1}\hspace{-0.7mm}\left(#2\right)}

\newcommand{\inlineqt}[2]{\left. #1 \!\middle/ #2 \right.}
\newcommand{\bigslant}[2]{{\left.\raisebox{.2em}{$#1$}\hspace{-1mm}\middle/\hspace{-0.7mm}\raisebox{-.2em}{$#2$}\right.}}

\newcommand{\probblock}[2]{\begin{shaded} \color{black} \textit{#1. #2}
\end{shaded} \color{black}}

\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\brackets}[1]{\left[#1\right]}
\newcommand{\brces}[1]{\left\{#1\right\}}


